Statistical Analysis and End-to-End Performance Evaluation of Traffic Models for Automotive Data

Autonomous driving is a major paradigm shift in transportation, with the potential to enhance safety, optimize traffic congestion, and reduce fuel consumption. Although autonomous vehicles rely on advanced sensors and on-board computing systems to navigate without human control, full awareness of the driving environment also requires a cooperative effort via Vehicle-To-Everything (V2X) communication. Specifically, vehicles send and receive sensor perceptions to/from other vehicles to extend perception beyond their own sensing range. However, transmitting large volumes of data can be challenging for current V2X communication technologies, so data compression represents a crucial solution to reduce the message size and link congestion. In this paper, we present a statistical characterization of automotive data, focusing on LiDAR sensors. Notably, we provide models for the size of both raw and compressed point clouds. The use of statistical traffic models offers several advantages compared to using real data, such as faster simulations, reduced storage requirements, and greater flexibility in the application design. Furthermore, statistical models can be used for understanding traffic patterns and analyzing statistics, which is crucial to design and optimize wireless networks. We validate our statistical models via a Kolmogorov-Smirnoff test implementing a Bootstrap Resampling scheme. Moreover, we show via ns-3 simulations that using statistical models yields comparable results in terms of latency and throughput compared to real data, which also demonstrates the accuracy of the models.

==> Figures/Tables/TaylorCoef.tex <==
\begin{tabular}{ll}
    \toprule
    \centering
    $i$ &  Coefficient\\
    \midrule
    1 & $1/ (6 * n) + 1.66\mathrm{e}{-1}$ \\
    2 & $5.8\mathrm{e}{-2}$ + (1/ ($1.5\mathrm{e}{1}$ * n)) + (1/ ($1.2\mathrm{e}{2}$ * $n^2$))  \\
    3 & $2.5\mathrm{e}{-2}$ + (3/ ($1.12\mathrm{e}{2}$ * n)) + (1/ ($5.6\mathrm{e}{2}$ * $n^2$)) + (1/ ($5.04\mathrm{e}{3}$  * $n^3$))  \\
    4 & $1.2\mathrm{e}{-2}$ + ($4.79\mathrm{e}{2}$/($4.53\mathrm{e}{3}$ * n)) - ($6.7\mathrm{e}{1}$/($6.04\mathrm{e}{4}$ *  $n^2$)) + (17/($4.53\mathrm{e}{4}$*  $n^3$))  + (1/($3.62\mathrm{e}{5}$*  $n^4$))  \\
    5 & $6.1\mathrm{e}{-3}$+ ($1.53\mathrm{e}{5}$/($3.99\mathrm{e}{7}$*n)) - ($1.28\mathrm{e}{3}$/($7.98\mathrm{e}{5}$*  $n^2$)) + ($1.18\mathrm{e}{4}$/ ($1.99\mathrm{e}{7}$ *  $n^3$)) - ($2.5\mathrm{e}{3}$/($3.99\mathrm{e}{7}$ *  $n^4$)) + (1/ ($3.99\mathrm{e}{7}$ *  $n^5$))  \\
    6 & $3.2\mathrm{e}{-3}$ + ($7.06\mathrm{e}{4}$/($6.48\mathrm{e}{7}$*n)) - ($8.70\mathrm{e}{5}$/($6.91\mathrm{e}{8}$* $n^2$)) + ($6.72\mathrm{e}{4}$/($9.72\mathrm{e}{7}$* $n^3$)) - 
    ($3.39\mathrm{e}{5}$/($2.07\mathrm{e}{9}$ * $n^4$)) \\ & + (37/($2.40\mathrm{e}{6}$ *  $n^5$)) + (1/($6.22\mathrm{e}{9}$ *  $n^6$)) \\
    7 &$1.74\mathrm{e}{-3}$ + ($4.38\mathrm{e}{7}$ / ($1.30\mathrm{e}{12}$*n)) - ($3.32\mathrm{e}{8}$/ ($4.35\mathrm{e}{11}$* $n^2$)) + ($8.43\mathrm{e}{8}$ / ($1.30\mathrm{e}{12}$*  $n^3$))- ($3.26\mathrm{e}{8}$/ ($1.30\mathrm{e}{12}$ *  $n^4$))\\ &
     + ($2.14\mathrm{e}{7}$/ ($4.35\mathrm{e}{11}$ *  $n^5$)) -($1.04\mathrm{e}{6}$/ ($2.61\mathrm{e}{11}$ *  $n^6$)) + (1/ ($1.30\mathrm{e}{12}$ *  $n^7$));  \\
    
     8 & $9.6\mathrm{e}{-4}$ - ($5.31\mathrm{e}{8}$/ ($1.71\mathrm{e}{12}$*n)) - ($3.22\mathrm{e}{10}$/ ($8.89\mathrm{e}{13}$* $n^2$)) + ($9.14\mathrm{e}{7}$/ ($1.77\mathrm{e}{11}$* $n^3$))  - ($5.18\mathrm{e}{10}$/ ($1.77\mathrm{e}{11}$* $n^4$))\\
     & + ($4.04\mathrm{e}{8}$/ ($4.44\mathrm{e}{12}$* $n^5$)) - ($1.23\mathrm{e}{8}$ /($8.08\mathrm{e}{12}$ *  $n^6$)) + ($2.42\mathrm{e}{7}$/ ($2.22\mathrm{e}{12}$ *  $n^7$)) + (1/($3.55\mathrm{e}{14}$ *  $n^8$))  \\
     9 & $5.4\mathrm{e}{-4}$ - ($1.49\mathrm{e}{13}$/ ($4.05\mathrm{e}{16}$*n)) - ($2.65\mathrm{e}{10}$/($2.59\mathrm{e}{14}$* $n^2$)) + ($7.39\mathrm{e}{10}$ / ($2.06\mathrm{e}{14}$ * $n^3$))  - ($5.81\mathrm{e}{12}$/($2.02\mathrm{e}{16}$*  $n^4$))\\
     & + ($4.49\mathrm{e}{10}$/ ($3.55\mathrm{e}{14}$*  $n^5$)) - ($1.76\mathrm{e}{8}$/($5.30\mathrm{e}{12}$* $n^6$)) + ($4.95\mathrm{e}{10}$/ ($1.01\mathrm{e}{16}$*  $n^7$)) - ($4.22\mathrm{e}{9}$ /($1.35\mathrm{e}{16}$* $n^8$)) + (1/($1.21\mathrm{e}{17}$ *  $n^9$))  \\
    
    \bottomrule
\end{tabular}

==> Figures/Tables/fitting_params.tex <==
\begin{tabular}{lllll}
    \toprule
    $m$ & Distribution $\mathbb{P}$ & Parameters & Values \\
    \midrule
    D0/S0 & tLocationScale & $\mu,\sigma,\nu$ & 3172.74, 64.41, 1.49 \\
    D0/S1 & Normal & $\mu,\sigma$ & 1458.7, 455.36 \\
    D0/S2 & Gamma & $a,b$ & 1.87, 131.97 \\
    D11/S0 & Nakagami & $\mu,\omega$ & 9.31, 4914.06 \\
    D14/S0 & Logistic & $\mu,\sigma$ & 197.54, 8.96 \\
    D14/S1 & tLocationScale & $\mu,\sigma,\nu$ & 98.11, 16.83, 4.08 \\
    D14/S2 & Gamma & $a, b$ & 2.81, 6.06 \\
    \bottomrule
\end{tabular}%
%
% Previous
%\begin{tabular}{lllll}
%    \toprule
%    $m$ & Distribution Name, $\mathbb{P}$ & Parameter Names, $\Theta$ & Parameter Values \\
%    \midrule
%    000 & tLocationScale & $\mu,\sigma,\nu$ & 3174.9238069608, 60.2675341943822, 1.5114792196029 \\
%    001 & Normal & $\mu,\sigma$ & 1468.58379378195, 442.196308024162 \\
%    002 & Gamma & $a,b$ & 1.87185305928113, 131.124782551148 \\
%    1150 & Nakagami & $\mu,\omega$ & 9.59199839942525, 4930.1644560103 \\
%    1450 & Logistic & $\mu,\sigma$ & 197.950686640472, 8.95410061800849 \\
%    1451 & tLocationScale & $\mu,\sigma,\nu$ & 98.6140292439172, 16.0475173490242, 4.10154896314596 \\
%    1452 & Nakagami & $\mu,\omega$ & 0.910148632299362, 381.858113512559 \\
%    \bottomrule
%\end{tabular}

==> Figures/Tables/pvalues.tex <==
\begin{tabular}{llllllll}
    \toprule
    $\mathbb{P}$ & D0/S0 & D0/S1 & D0/S2 & D11/S0 & D14/S0 & D14/S1 & D14/S2 \\
    \midrule
        BirnbaumSaunders & 0 & 0.0 & \textbf{0.061} & \textbf{0.013} & 0.0 & 0.0 & 0.0 \\
        ExtremeValue & 0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.003 & 0.0 \\
        Gamma & 0 & 0.0 & \cellcolor{black!15}\textbf{0.375} & \textbf{0.114} & 0.0 & 0.0 & \cellcolor{black!15}\textbf{0.012} \\
        GeneralizedExtremeValue & 0 & 0.003 & \textbf{0.039} & 0.006 & 0.0 & 0.0 & 0.0 \\
        HalfNormal & 0 & 0.0 & 0.003 & 0.0 & 0.0 & 0.0 & 0.0 \\
        InverseGaussian & 0 & 0.0 & 0.002 & \textbf{0.018} & 0.0 & 0.0 & 0.0 \\
        Logistic & 0 & 0.009 & 0.0 & 0.0 & \cellcolor{black!15}\textbf{0.036} & \textbf{0.024} & 0.0 \\
        Loglogistic & 0 & 0.0 & \textbf{0.018} & \textbf{0.037} & 0.01 & 0.0 & 0.0 \\
        Lognormal & 0 & 0.0 & \textbf{0.065} & \textbf{0.02} & 0.0 & 0.0 & 0.0 \\
        Nakagami & 0 & 0.001 & 0.0 & \cellcolor{black!15}\textbf{0.128} & 0.0 & 0.0 & 0.004 \\
        Normal & 0 & \cellcolor{black!15}\textbf{0.109} & 0.0 & \textbf{0.012} & 0.0 & 0.0 & 0.0 \\
        Poisson & 0 & 0.0 & 0.0 & 0.0 & 0.007 & 0.0 & 0.0 \\
        Rayleigh & 0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
        tLocationScale & \cellcolor{black!15}0 & \textbf{0.029} & 0.0 & \textbf{0.014} & \textbf{0.026} & \cellcolor{black!15}\textbf{0.026} & 0.0 \\
        Weibull & 0 & \textbf{0.044} & \textbf{0.15} & 0.0 & 0.003 & 0.0 & 0.01 \\
    \bottomrule
\end{tabular}


==> Figures/acronyms.tex <==
\newacronym{quic}{QUIC}{Quick UDP Internet Connections}
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{adc}{ADC}{Analog to Digital Converter}
\newacronym{5g}{5G}{5th Generation}
\newacronym{aimd}{AIMD}{Additive Increase Multiplicative Decrease}
\newacronym{am}{AM}{Acknowledged Mode}
\newacronym{amc}{AMC}{Adaptive Modulation and Coding}
\newacronym{aqm}{AQM}{Active Queue Management}
\newacronym{awgn}{AGWN}{Additive White Gaussian Noise}
\newacronym{balia}{BALIA}{Balanced Link Adaptation}
\newacronym{bdp}{BDP}{Bandwidth-Delay Product}
\newacronym{bf}{BF}{Beamforming}
\newacronym{cc}{CC}{Congestion Control}
\newacronym{pdf}{PDF}{Probability Density Function}
\newacronym{cdf}{CDF}{Cumulative Distribution Function}
\newacronym{icdf}{Inverse CDF}{Inverse Cumulative Distribution Function}
\newacronym{c-v2x}{C-V2X}{Cellular Vehicle-To-Everything}
\newacronym{ci}{CI}{Close-in free space reference}
\newacronym{cn}{CN}{Core Network}
\newacronym{cqi}{CQI}{Channel Quality Information}
\newacronym{cp}{CP}{Control Plane}
\newacronym{csirs}{CSI-RS}{Channel State Information - Reference Signal}
\newacronym{d2d}{D2D}{Device-to-Device}
\newacronym{dc}{DC}{Dual Connectivity}
\newacronym{mle}{MLE}{Maximum Likelihood Estimation}
\newacronym{dce}{DCE}{Direct Code Execution}
\newacronym{dci}{DCI}{Downlink Control Information}
%\newacronym{dl}{DL}{Downlink}
\newacronym{dmr}{DMR}{Deadline Miss Ratio}
\newacronym{dmrs}{DMRS}{DeModulation Reference Signal}
\newacronym{dsrc}{DSRC}{Dedicated Short-Range Communication}
\newacronym{e2e}{E2E}{End-to-End}
\newacronym{ecn}{ECN}{Explicit Congestion Notification}
\newacronym{edf}{EDF}{Earliest Deadline First}
\newacronym{enb}{eNB}{evolved Node Base}
\newacronym{epc}{EPC}{Evolved Packet Core}
\newacronym{es}{ES}{Edge Server}
\newacronym{fdma}{FDMA}{Frequency Division Multiple Access}
\newacronym{fdd}{FDD}{Frequency Division Duplexing}
\newacronym[firstplural=Radio Access Technologies (RATs)]{rat}{RAT}{Radio Access Technology}
\newacronym{fs}{FS}{Fast Switching}
\newacronym{ftp}{FTP}{File Transfer Protocol}
\newacronym{gnb}{gNB}{Next Generation Node Base}
\newacronym{harq}{HARQ}{Hybrid Automatic Repeat reQuest}
\newacronym{hetnet}{HetNet}{Heterogeneous Network}
\newacronym{hh}{HH}{Hard Handover}
\newacronym{hol}{HOL}{Head-of-Line}
\newacronym{ia}{IA}{Initial Access}
\newacronym{imt}{IMT}{International Mobile Telecommunication}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{lidar}{LiDAR}{Light Detection and Ranging}
\newacronym{los}{LoS}{Line of Sight}
\newacronym{lstm}{LSTM}{long short-term memory}
\newacronym{lte}{LTE}{Long Term Evolution}
\newacronym{m2m}{M2M}{Machine-to-Machine}
\newacronym{mac}{MAC}{Medium Access Control}
\newacronym{mc}{MC}{Multi-Connectivity}
\newacronym{mcs}{MCS}{Modulation and Coding Scheme}
\newacronym{mec}{MEC}{Mobile Edge Cloud}
\newacronym{mi}{MI}{Mutual Information}
\newacronym{mimo}{MIMO}{Multiple Input, Multiple Output}
\newacronym{mmwave}{mmWave}{millimeter wave}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{mpc}{MPC}{Model Predictive Control}
\newacronym{mr}{MR}{Maximum Rate}
\newacronym{mss}{MSS}{Maximum Segment Size}
\newacronym{mtd}{MTD}{Machine-Type Device}
\newacronym{mtu}{MTU}{Maximum Transmission Unit}
\newacronym{nn}{NN}{Neural Network}
\newacronym{nsf}{NSF}{National Science Foundation}
\newacronym{nfv}{NFV}{Network Function Virtualization}
\newacronym{nlos}{nLoS}{non-Line-of-Sight}
\newacronym{nr}{NR}{New Radio}
\newacronym{ofdm}{OFDM}{Orthogonal Frequency Division Multiplexing}
\newacronym{pc}{PC}{Point Cloud}
\newacronym{pdcch}{PDCCH}{Physical Downlonk Control Channel}
\newacronym{pdcp}{PDCP}{Packet Data Convergence Protocol}
\newacronym{pdsch}{PDSCH}{Physical Downlink Shared Channel}
\newacronym{pdu}{PDU}{Packet Data Unit}
\newacronym{pf}{PF}{Proportional Fair}
\newacronym{pgw}{PGW}{Packet Gateway}
\newacronym{phy}{PHY}{Physical}
\newacronym{pbch}{PBCH}{Physical Broadcast Channel}
\newacronym[plural=\gls{mme}s,firstplural=Mobility Management Entities (MMEs)]{mme}{MME}{Mobility Management Entity}
\newacronym{prb}{PRB}{Physical Resource Block}
\newacronym{pss}{PSS}{Primary Synchronization Signal}
\newacronym{pucch}{PUCCH}{Physical Uplink Control Channel}
\newacronym{pusch}{PUSCH}{Physical Uplink Shared Channel}
\newacronym{qos}{QOS}{Quality of Service}
\newacronym{rach}{RACH}{Random Access Channel}
\newacronym{ran}{RAN}{Radio Access Network}
\newacronym{red}{RED}{Random Early Detection}
\newacronym{rf}{RF}{Radio Frequency}
\newacronym{rlc}{RLC}{Radio Link Control}
\newacronym{rlf}{RLF}{Radio Link Failure}
\newacronym{rrc}{RRC}{Radio Resource Control}
\newacronym{rrm}{RRM}{Radio Resource Management}
\newacronym{rr}{RR}{Round Robin}
\newacronym{rs}{RS}{Remote Server}
\newacronym{rsrp}{RSRP}{Reference Signal Received Power}
\newacronym{rss}{RSS}{Received Signal Strength}
\newacronym{rtt}{RTT}{Round Trip Time}
\newacronym{rw}{RW}{Receive Window}
\newacronym{rx}{RX}{Receiver}
\newacronym{sa}{SA}{standalone}
\newacronym{sack}{SACK}{Selective Acknowledgment}
\newacronym{sap}{SAP}{Service Access Point}
\newacronym{sch}{SCH}{Secondary Cell Handover}
\newacronym{scoot}{SCOOT}{Split Cycle Offset Optimization Technique}
\newacronym{sdma}{SDMA}{Spatial Division Multiple Access}
\newacronym{sinr}{SINR}{Signal to Interference plus Noise Ratio}
\newacronym{sm}{SM}{Saturation Mode}
\newacronym{snr}{SNR}{Signal to Noise Ratio}
\newacronym{psnr}{PSNR}{Peak Signal to Noise Ratio}
\newacronym{son}{SON}{Self-Organizing Network}
\newacronym{ss}{SS}{Synchronization Signal}
\newacronym{srs}{SRS}{Sounding Reference Signal}
\newacronym{sss}{SSS}{Secondary Synchronization Signal}
\newacronym{tb}{TB}{Transport Block}
\newacronym{tcp}{TCP}{Transmission Control Protocol}
\newacronym{tdd}{TDD}{Time Division Duplexing}
\newacronym{tdma}{TDMA}{Time Division Multiple Access}
\newacronym{tfl}{TfL}{Transport for London}
\newacronym{thz}{THz}{Terahertz}
\newacronym{tm}{TM}{Transparent Mode}
\newacronym{trp}{TRP}{Transmitter Receiver Pair}
\newacronym{tti}{TTI}{Transmission Time Interval}
\newacronym{ttt}{TTT}{Time-to-Trigger}
\newacronym{tx}{TX}{Transmitter}
\newacronym{ue}{UE}{User Equipment}
\newacronym{ul}{UL}{Uplink}
\newacronym{uml}{UML}{Unified Modeling Language}
\newacronym{um}{UM}{Unacknowledged Mode}
\newacronym{utc}{UTC}{Urban Traffic Control}
\newacronym{v2i}{V2I}{Vehicle-to-Infrastructure}
\newacronym{v2v}{V2V}{Vehicle-to-Vehicle}
\newacronym{vm}{VM}{Virtual Machine}
\newacronym{rsrq}{RSRQ}{Reference Signal Received Quality}
\newacronym{rssi}{RSSI}{Received Signal Strength Indicator}
\newacronym{crs}{CRS}{Cell Reference Signal}
\newacronym{comp}{CoMP}{Coordinated Multi-Point}
\newacronym{cran}{C-RAN}{Cloud \acrlong{ran}}
\newacronym{ca}{CA}{Carrier Aggregation}
\newacronym{cco}{CC}{Carrier Component}
\newacronym{nsa}{NSA}{Non Stand Alone}
\newacronym{embb}{eMBB}{Enhanced Mobility Broadband}
\newacronym{bsr}{BSR}{Buffer Status Report}
\newacronym{srb}{SRB}{Service Radio Bearer}
\newacronym{scm}{SCM}{Spatial Channel Model}
\newacronym{sctp}{SCTP}{Stream Control Transmission Protocol}
\newacronym{mptcp}{MPTCP}{Multi-path TCP}
\newacronym{ietf}{IETF}{Internet Engineering Task Force}
\newacronym{os}{OS}{Operating System}
\newacronym{tls}{TLS}{Transport Layer Security}
\newacronym{rfc}{RFC}{Request for Comments}
\newacronym{http}{HTTP}{HyperText Transfer Protocol}
\newacronym{nat}{NAT}{Network Address Translation}
\newacronym{api}{API}{Application Programming Interface}
\newacronym{rto}{RTO}{Retransmission Timeout}
\newacronym{psc}{PSC}{Public Safety Communication}
\newacronym{rpgm}{RPGM}{Reference Point Group Mobility}
\newacronym{ic}{IC}{Incident Command}
\newacronym{rsu}{RSU}{Road Side Unit}
\newacronym{uav}{UAV}{Unmanned Aerial Vehicle}
\newacronym{usa}{U.S.}{United States}
\newacronym{vr}{VR}{Virtual Reality}
\newacronym{iab}{IAB}{Integrated Access and Backhaul}
\newacronym{wlan}{WLAN}{Wireless Local Area Network}
\newacronym{cots}{COTS}{Commercial Off-the-Shelf}
\newacronym{fpga}{FPGA}{Field Programmable Gate Array}
\newacronym{rcn}{RCN}{Research Coordination Network}
\newacronym{abg}{ABG}{Alpha-Beta-Gamma}
\newacronym{fi}{FI}{Floating Intercept}
\newacronym{uas}{UAS}{Unmanned Aerial System}
\newacronym{gps}{GPS}{Global Positioning System}
\newacronym{a2g}{A2G}{air-to-ground}
\newacronym{a2a}{A2A}{air-to-air}
\newacronym{uma}{UMa}{Urban Macro}
\newacronym{umi}{UMi}{Urban Micro}
\newacronym{upa}{UPA}{Uniform Planar Array}
\newacronym{rma}{RMa}{Rural Macro}
\newacronym{inoo}{InOo}{Indoor Open Office}
\newacronym{ple}{PLE}{path loss exponent}
\newacronym{aoa}{AoA}{Angle of Arrival}
\newacronym{aod}{AoD}{Angle of Departure}
\newacronym{toa}{ToA}{Time of Arrival}
% \newacronym{mpc}{MPC}{Multi-path Component}
\newacronym{cir}{CIR}{Channel Impulse Response}
\newacronym{rt}{RT}{Ray-tracing}
\newacronym{tc}{TC}{Time Cluster}
\newacronym{svd}{SVD}{Singular Value Decomposition}
\newacronym{6g}{6G}{sixth generation}
\newacronym{ns3}{ns-3}{Network Simulator 3}
\newacronym{fsc}{FS}{Fully Stochastic}
\newacronym{hbc}{HB}{Hybrid}
\newacronym{hpbw}{HPBW}{Half Power Beamwidth}
\newacronym{hsc}{HSC}{Hybrid Semantic Compression}
\newacronym{prr}{PRR}{Packet Receipt Rate}
\newacronym{v2x}{V2X}{Vehicle-To-Everything}
\newacronym{dl}{DL}{Deep Learning}
\newacronym{cl}{CL}{Compression Level}
\newacronym{sl}{SL}{Semantic Level}
\newacronym{qp}{QP}{Quantization Parameter}
\newacronym{p2pPSNR}{p2p-PSNR}{Point-to-Plane PSNR}
\newacronym{p2p}{P2P}{Peer-to-Peer}
\newacronym{xr}{XR}{eXtended Reality}
\newacronym{hmd}{HMD}{Head Mounted Device}
\newacronym{ks}{KS}{Kolmogorov-Smirnoff}
\newacronym{nrmse}{NRMSE}{Normalized Root Mean Squared Error}

